A Closer Look at Few-Shot Crosslingual Transfer: The Choice of Shots Matters

Few-shot crosslingual transfer has been shown to outperform its zero-shot counterpart with pretrained encoders like multilingual BERT. Despite its growing popularity, little to no attention has been paid to standardizing and analyzing the design of few-shot experiments. In this work, we highlight a fundamental risk posed by this shortcoming, illustrating that the model exhibits a high degree of sensitivity to the selection of few shots. We conduct a large-scale experimental study on 40 sets of sampled few shots for six diverse NLP tasks across up to 40 languages. We provide an analysis of success and failure cases of few-shot transfer, which highlights the role of lexical features. Additionally, we show that a straightforward full model finetuning approach is quite effective for few-shot transfer, outperforming several state-of-the-art few-shot approaches. As a step towards standardizing few-shot crosslingual experimental designs, we make our sampled few shots publicly available.

==> cvclstable.tex <==
\begin{table}[!]
  \centering
  \tiny
  \def\arraystretch{0.93}  
  \setlength{\tabcolsep}{4pt}   
  \begin{tabular}{cc|ccccc}
                   &    & K=0   & K=1              & K=2              & K=4              & K=8              \\ \hline
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{MLDoc}}} & EN & 96.88 & -                & -                & -                & -                \\
                   & DE & 88.30 & \BC{90.13 $\pm$ 1.37} & \BC{90.69 $\pm$ 1.01} & \BC{91.72 $\pm$ 0.78} & \BC{91.94 $\pm$ 0.73} \\
                   & FR & 83.05 & \BC{88.46 $\pm$ 2.40} & \BC{89.24 $\pm$ 1.88} & \BC{90.84 $\pm$ 0.86} & \BC{90.87 $\pm$ 1.01} \\
                   & ES & 81.90 & \BC{83.18 $\pm$ 2.53} & \BC{85.45 $\pm$ 1.80} & \BC{86.04 $\pm$ 2.03} & \BC{88.39 $\pm$ 1.84} \\
                   & IT & 74.13 & \BC{74.84 $\pm$ 1.94} & \BC{75.18 $\pm$ 1.57} & \BC{76.38 $\pm$ 1.40} & \BC{78.30 $\pm$ 1.25} \\
                   & RU & 72.33 & \BC{77.04 $\pm$ 4.34} & \BC{79.20 $\pm$ 2.87} & \BC{80.51 $\pm$ 2.67} & \BC{81.82 $\pm$ 1.24} \\
                   & ZH & 84.38 & \BC{86.71 $\pm$ 1.82} & \BC{86.58 $\pm$ 1.67} & \BC{87.83 $\pm$ 1.12} & \BC{88.63 $\pm$ 1.08} \\
                   & JA & 74.58 & \BC{75.76 $\pm$ 1.83} & \BC{76.74 $\pm$ 2.08} & \BC{78.50 $\pm$ 2.33} & \BC{81.22 $\pm$ 1.82} \\ \hline\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{MARC}}} & EN & 64.52 & -                & -                & -                & -                \\
                   & DE & 49.62 & \BC{50.48 $\pm$ 2.00} & \BC{52.31 $\pm$ 0.95} & \BC{52.44 $\pm$ 1.04} & \BC{53.16 $\pm$ 0.63} \\
                   & FR & 47.30 & \BC{49.15 $\pm$ 1.45} & \BC{49.25 $\pm$ 1.31} & \BC{50.63 $\pm$ 1.03} & \BC{51.03 $\pm$ 0.83} \\
                   & ES & 48.44 & \BC{48.72 $\pm$ 1.53} & \BC{49.66 $\pm$ 1.13} & \BC{50.08 $\pm$ 1.19} & \BC{51.08 $\pm$ 0.94} \\
                   & ZH & 40.40 & \BC{42.55 $\pm$ 2.51} & \BC{43.71 $\pm$ 1.65} & \BC{44.89 $\pm$ 1.36} & \BC{45.99 $\pm$ 1.17} \\
                   & JA & 38.84 & \BC{40.62 $\pm$ 2.61} & \BC{43.10 $\pm$ 1.32} & \BC{43.67 $\pm$ 1.07} & \BC{44.38 $\pm$ 0.67} \\ \hline\hline
\multirow{15}{*}{\rotatebox[origin=c]{90}{\textbf{XNLI}}} & EN & 82.67 & -                &    -             &    -             &    -             \\
                   & DE & 70.32 & \WC{70.23 $\pm$ 0.92} & \WC{69.83 $\pm$ 0.95} & \BC{70.42 $\pm$ 0.51} & \BC{70.59 $\pm$ 0.40} \\
                   & FR & 73.57 & \WC{72.33 $\pm$ 1.72} & \WC{73.48 $\pm$ 0.54} & \WC{73.46 $\pm$ 0.71} & \BC{73.60 $\pm$ 0.89} \\
                   & ES & 73.71 & \WC{73.33 $\pm$ 0.82} & \WC{73.64 $\pm$ 0.58} & \WC{73.58 $\pm$ 0.56} & \BC{73.85 $\pm$ 0.47} \\
                   & RU & 68.70 & \WC{66.15 $\pm$ 2.53} & \WC{68.63 $\pm$ 0.62} & \BC{68.78 $\pm$ 0.44} & \BC{68.81 $\pm$ 0.48} \\
                   & ZH & 69.32 & \WC{69.10 $\pm$ 1.21} & \WC{68.19 $\pm$ 2.26} & \BC{70.39 $\pm$ 0.85} & \BC{70.61 $\pm$ 0.89} \\
                   & AR & 64.97 & \WC{64.32 $\pm$ 1.13} & \WC{64.33 $\pm$ 0.67} & \WC{64.54 $\pm$ 0.57} & \WC{64.88 $\pm$ 0.37} \\
                   & BG & 67.58 & \BC{67.58 $\pm$ 0.96} & \BC{67.65 $\pm$ 1.12} & \BC{68.10 $\pm$ 1.02} & \BC{68.27 $\pm$ 0.63} \\
                   & EL & 65.67 & \WC{64.53 $\pm$ 1.50} & \WC{65.31 $\pm$ 0.97} & \BC{65.72 $\pm$ 0.61} & \BC{65.87 $\pm$ 0.51} \\
                   & HI & 56.57 & \WC{55.66 $\pm$ 1.95} & \WC{55.81 $\pm$ 1.97} & \BC{57.06 $\pm$ 1.09} & \BC{57.56 $\pm$ 1.42} \\
                   & SW & 48.08 & \BC{49.57 $\pm$ 2.16} & \BC{49.74 $\pm$ 1.53} & \BC{50.77 $\pm$ 0.78} & \BC{51.32 $\pm$ 0.61} \\
                   & TH & 46.17 & \BC{48.63 $\pm$ 3.07} & \BC{49.50 $\pm$ 2.79} & \BC{50.76 $\pm$ 2.53} & \BC{52.10 $\pm$ 2.60} \\
                   & TR & 60.40 & \BC{60.40 $\pm$ 0.92} & \WC{59.01 $\pm$ 2.00} & \BC{60.63 $\pm$ 0.98} & \BC{61.42 $\pm$ 0.54} \\
                   & UR & 57.05 & \WC{56.81 $\pm$ 1.38} & \BC{57.46 $\pm$ 1.47} & \BC{58.11 $\pm$ 1.06} & \BC{58.46 $\pm$ 0.80} \\
                   & VI & 69.82 & \WC{68.94 $\pm$ 1.47} & \WC{69.62 $\pm$ 0.98} & \BC{70.17 $\pm$ 0.74} & \BC{70.07 $\pm$ 0.92} \\ \hline\hline
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{PAWSX}}}   & EN & 93.90 & -                & -                & -                & -                  \\
                  & DE & 83.80 & \WC{83.23 $\pm$ 1.14} & \WC{83.40 $\pm$ 1.00} & \WC{83.40 $\pm$ 1.07} & \BC{83.82 $\pm$ 1.02}   \\
                  & FR & 86.90 & \WC{86.53 $\pm$ 1.11} & \WC{86.57 $\pm$ 0.83} & \WC{86.45 $\pm$ 0.69} & \BC{86.90 $\pm$ 0.42}   \\
                  & ES & 88.25 & \WC{87.20 $\pm$ 1.29} & \WC{87.75 $\pm$ 0.61} & \WC{87.79 $\pm$ 0.50} & \WC{87.71 $\pm$ 0.78}   \\
                  & ZH & 77.75 & \WC{76.73 $\pm$ 1.99} & \WC{77.28 $\pm$ 0.77} & \WC{77.44 $\pm$ 0.75} & \BC{77.86 $\pm$ 0.68}   \\
                  & JA & 73.30 & \BC{73.31 $\pm$ 1.29} & \BC{73.31 $\pm$ 0.74} & \BC{73.52 $\pm$ 0.66} & \BC{74.04 $\pm$ 1.11}   \\    
                  & KO & 72.05 & \WC{72.01 $\pm$ 1.83} & \BC{73.53 $\pm$ 1.47} & \BC{73.37 $\pm$ 1.11} & \BC{73.81 $\pm$ 1.03} \\

  \end{tabular}
  \caption{Zero- (column K=0) and few- (columns K$>$0) shot transfer results (\%)
    on the test set of CLS tasks: MLDoc, MARC, XNLI, and PAWSX, when using small dev set.
    Green [red]:  few-shot transfer outperforms [underperforms] zero-shot transfer.}
  \tablabel{CVbigclstable}
\end{table}



==> mldocmarcfewshottable.tex <==
\begin{table}[t]
  \centering
  \tiny
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{c|ccccc}
       & K=0   & K=1              & K=2              & K=4              & K=8              \\ \hline
    EN & 96.88 & -                & -                & -                & -                \\
    DE & 88.30 & 90.36 $\pm$ 1.48 & 90.77 $\pm$ 0.87 & 91.85 $\pm$ 0.83 & 91.98 $\pm$ 0.82 \\
    FR & 83.05 & 88.94 $\pm$ 2.46 & 89.71 $\pm$ 1.68 & 90.80 $\pm$ 0.88 & 91.01 $\pm$ 0.94 \\
    ES & 81.90 & 83.99 $\pm$ 2.35 & 85.65 $\pm$ 1.60 & 86.30 $\pm$ 1.85 & 88.46 $\pm$ 1.90 \\
    IT & 74.13 & 74.97 $\pm$ 2.04 & 75.29 $\pm$ 1.57 & 76.43 $\pm$ 1.41 & 78.12 $\pm$ 1.25 \\
    RU & 72.33 & 77.40 $\pm$ 4.27 & 80.57 $\pm$ 1.37 & 81.33 $\pm$ 1.33 & 81.91 $\pm$ 1.21 \\
    ZH & 84.38 & 87.18 $\pm$ 1.45 & 87.31 $\pm$ 1.53 & 88.33 $\pm$ 1.11 & 88.72 $\pm$ 1.05 \\
    JA & 74.58 & 76.23 $\pm$ 1.59 & 76.71 $\pm$ 2.12 & 78.60 $\pm$ 2.43 & 81.17 $\pm$ 1.72 \\ \hline\hline
    EN & 64.52 & -                & -                & -                & -                \\
    DE & 49.62 & 51.50 $\pm$ 1.58 & 52.76 $\pm$ 0.87 & 52.78 $\pm$ 1.00 & 53.32 $\pm$ 0.59 \\
    FR & 47.30 & 49.32 $\pm$ 1.34 & 49.70 $\pm$ 1.43 & 50.64 $\pm$ 0.94 & 51.23 $\pm$ 0.76 \\
    ES & 48.44 & 49.72 $\pm$ 1.24 & 49.96 $\pm$ 1.12 & 50.45 $\pm$ 1.22 & 51.25 $\pm$ 0.93 \\
    ZH & 40.40 & 43.19 $\pm$ 1.76 & 44.45 $\pm$ 1.36 & 45.40 $\pm$ 1.26 & 46.40 $\pm$ 0.93 \\
    JA & 38.84 & 41.95 $\pm$ 2.09 & 43.63 $\pm$ 1.30 & 43.98 $\pm$ 0.89 & 44.44 $\pm$ 0.69
  \end{tabular}
  \caption{Zero-shot (column K=0) and few-shot (columns K$>$0) crosslingual transfer results
    on the test
    set of MLDoc (top) and MARC (bottom). }
  \tablabel{mldocmarcfewshot}
\end{table}



==> posnerfewshottable.tex <==
\begin{table*}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{1.0pt}
  \renewcommand{\arraystretch}{1.1}
  \begin{tabularx}{\textwidth}{@{}l XXXX XXXX}
                & \multicolumn{4}{c}{\textsc{NER}} & \multicolumn{4}{c}{\textsc{POS}}                                                                              \\
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
                & K=0         & K=1               & K=2             & K=4              & K=0   & K=1              & K=2              & K=4              \\
    \textsc{en} & 83.65       & -                 & -               & -                & 95.39 & -                & -                & -                \\
    \textsc{af} & 78.36       & 79.07 $\pm$ 1.47  &79.69 $\pm$ 1.40 &80.24 $\pm$ 1.16  & 86.60 & 91.10 $\pm$ 1.11 & 92.12 $\pm$ 1.15 & 93.50 $\pm$ 0.56 \\
    \textsc{ar} & 39.91       & 54.44 $\pm$ 6.74  &60.51 $\pm$ 4.30 &63.61 $\pm$ 2.65  & 66.55 & 75.64 $\pm$ 1.09 & 77.01 $\pm$ 0.84 & 78.52 $\pm$ 0.67 \\
    \textsc{bg} & 78.59       & 78.65 $\pm$ 0.38  &78.70 $\pm$ 0.39 &78.87 $\pm$ 0.48  & 87.02 & 91.01 $\pm$ 0.97 & 91.97 $\pm$ 0.90 & 93.18 $\pm$ 0.56 \\
    \textsc{bn} & 64.17       & 66.37 $\pm$ 1.69  &66.66 $\pm$ 1.57 &65.98 $\pm$ 2.11  & -     & -               & -               & -    \\
    \textsc{de} & 79.00       & 79.33 $\pm$ 0.71  &79.61 $\pm$ 0.76 &79.74 $\pm$ 0.73  & 86.38 & 89.38 $\pm$ 0.90 & 90.21 $\pm$ 0.50 & 91.32 $\pm$ 0.43 \\
    \textsc{el} & 75.20       & 74.93 $\pm$ 0.79  &75.18 $\pm$ 0.95 &75.40 $\pm$ 0.93 & 81.89 & 89.69 $\pm$ 1.05 & 90.53 $\pm$ 0.89 & 91.58 $\pm$ 0.72 \\
    \textsc{es} & 77.16       & 79.19 $\pm$ 1.97  &80.28 $\pm$ 1.71 &80.90 $\pm$ 1.94  & 86.64 & 90.05 $\pm$ 1.01 & 91.19 $\pm$ 0.74 & 92.31 $\pm$ 0.52 \\
    \textsc{et} & 71.88       & 72.58 $\pm$ 1.17  &73.60 $\pm$ 1.65 &74.60 $\pm$ 1.59  & 79.17 & 81.69 $\pm$ 1.09 & 83.05 $\pm$ 0.98 & 84.39 $\pm$ 0.56 \\
    \textsc{eu} & 55.35       & 59.60 $\pm$ 3.32  &61.59 $\pm$ 3.84 &64.68 $\pm$ 2.96  & 49.51 & 68.44 $\pm$ 2.47 & 71.94 $\pm$ 1.78 & 75.89 $\pm$ 1.20 \\
    \textsc{fa} & 40.73       & 59.20 $\pm$ 5.34  &68.55 $\pm$ 4.04 &71.13 $\pm$ 3.45  & 65.73 & 80.82 $\pm$ 2.14 & 82.81 $\pm$ 1.79 & 84.95 $\pm$ 1.16 \\
    \textsc{fi} & 68.43       & 71.43 $\pm$ 2.61  &73.92 $\pm$ 2.44 &75.81 $\pm$ 2.15  & 74.49 & 78.25 $\pm$ 1.22 & 79.65 $\pm$ 0.85 & 81.32 $\pm$ 0.82 \\
    \textsc{fr} & 80.38       & 80.54 $\pm$ 0.93  &81.08 $\pm$ 0.85 &81.22 $\pm$ 0.93  & 82.54 & 89.55 $\pm$ 1.08 & 90.84 $\pm$ 0.64 & 91.66 $\pm$ 0.60 \\
    \textsc{he} & 56.36       & 58.24 $\pm$ 2.25  &59.43 $\pm$ 2.29 &60.27 $\pm$ 2.43  & 76.79 & 80.40 $\pm$ 1.42 & 82.42 $\pm$ 1.06 & 83.98 $\pm$ 0.83 \\
    \textsc{hi} & 65.84       & 67.16 $\pm$ 1.61  &67.56 $\pm$ 2.18 &68.29 $\pm$ 1.76  & 64.29 & 78.87 $\pm$ 1.26 & 80.80 $\pm$ 0.80 & 81.97 $\pm$ 0.92 \\
    \textsc{hu} & 71.28       & 72.23 $\pm$ 1.33  &73.03 $\pm$ 1.44 &74.14 $\pm$ 1.61  & 75.10 & 84.44 $\pm$ 1.40 & 86.31 $\pm$ 0.90 & 88.61 $\pm$ 0.67 \\
    \textsc{id} & 60.10       & 77.87 $\pm$ 6.31  &78.57 $\pm$ 4.14 &81.07 $\pm$ 1.50  & 70.80 & 72.68 $\pm$ 1.08 & 73.64 $\pm$ 0.78 & 74.34 $\pm$ 0.75\\
    \textsc{it} & 80.30       & 80.68 $\pm$ 0.79  &81.00 $\pm$ 0.92 &80.90 $\pm$ 1.12  & 85.97 & 88.77 $\pm$ 0.87 & 89.93 $\pm$ 0.50 & 90.77 $\pm$ 0.59\\
    \textsc{ja} & 7.16        & 20.71 $\pm$ 7.07  &28.23 $\pm$ 5.32 &32.93 $\pm$ 6.03  & 47.60 & 75.84 $\pm$ 1.68 & 78.46 $\pm$ 1.31 & 80.42 $\pm$ 0.98 \\
    \textsc{jv} & 61.18       & 67.80 $\pm$ 4.72  &69.79 $\pm$ 3.37 &72.12 $\pm$ 3.34  & -     & -               & -               & -    \\
    \textsc{ka} & 61.26       & 61.62 $\pm$ 1.09  &62.25 $\pm$ 1.56 &63.68 $\pm$ 1.66  & -     & -               & -               & -    \\
    \textsc{kk} & 40.29       & 50.42 $\pm$ 5.49  &54.97 $\pm$ 6.81 &62.94 $\pm$ 4.55  & -     & -               & -               & -    \\
    \textsc{ko} & 46.50       & 47.25 $\pm$ 1.36  &48.69 $\pm$ 1.82 &51.76 $\pm$ 2.30  & 42.29 & 57.43 $\pm$ 1.36 & 59.92 $\pm$ 1.18 & 62.37 $\pm$ 1.22 \\
    \textsc{ml} & 46.77       & 47.83 $\pm$ 2.30  &49.51 $\pm$ 3.01 &51.41 $\pm$ 3.31  & -     & -               & -               & -    \\
    \textsc{mr} & 54.70       & 55.78 $\pm$ 2.54  &57.22 $\pm$ 2.43 &59.18 $\pm$ 3.13  & 58.70 & 71.60 $\pm$ 2.52 & 74.89 $\pm$ 1.95 & 77.21 $\pm$ 1.77 \\
    \textsc{ms} & 68.61       & 71.04 $\pm$ 3.07  &74.51 $\pm$ 4.28 &76.25 $\pm$ 3.04  & -     & -               & -               & -    \\
    \textsc{my} & 42.45       & 43.55 $\pm$ 3.88  &46.03 $\pm$ 4.48 &47.81 $\pm$ 4.28  & -     & -               & -               & -    \\
    \textsc{nl} & 82.77       & 82.73 $\pm$ 0.43  &82.83 $\pm$ 0.54 &82.82 $\pm$ 0.46  & 88.35 & 88.97 $\pm$ 0.73 & 89.55 $\pm$ 0.79 & 90.83 $\pm$ 0.54 \\
    \textsc{pt} & 79.28       & 79.89 $\pm$ 0.99  &80.39 $\pm$ 0.98 &80.49 $\pm$ 0.95  & 86.45 & 88.18 $\pm$ 0.70 & 88.98 $\pm$ 0.66 & 89.78 $\pm$ 0.38\\
    \textsc{ru} & 65.20       & 67.30 $\pm$ 2.38  &68.78 $\pm$ 2.73 &71.34 $\pm$ 2.82  & 86.36 & 89.07 $\pm$ 0.76 & 89.85 $\pm$ 0.57 & 91.13 $\pm$ 0.51  \\
    \textsc{sw} & 68.36       & 71.07 $\pm$ 4.28  &70.08 $\pm$ 3.15 &74.33 $\pm$ 5.25  & -     & -               & -               & -    \\
    \textsc{ta} & 46.12       & 47.81 $\pm$ 1.81  &49.86 $\pm$ 2.99 &52.23 $\pm$ 2.63  & 53.51 & 62.84 $\pm$ 2.69 & 66.30 $\pm$ 1.56 & 69.36 $\pm$ 1.13 \\
    \textsc{te} & 50.02       & 52.57 $\pm$ 1.91  &54.02 $\pm$ 2.65 &55.75 $\pm$ 2.72  & 67.48 & 71.46 $\pm$ 2.58 & 75.72 $\pm$ 1.94 & 78.84 $\pm$ 1.44 \\
    \textsc{th} & 1.53        & 4.56 $\pm$ 4.87   &6.08 $\pm$ 4.88  &5.87 $\pm$ 4.14   & -     &  -              &  -              &  -   \\
    \textsc{tl} & 69.23       & 72.34 $\pm$ 2.25  &72.63 $\pm$ 2.43 &73.55 $\pm$ 2.25  & -     &  -              &  -              &  -   \\
    \textsc{tr} & 65.78       & 69.37 $\pm$ 2.24  &69.53 $\pm$ 2.07 &72.33 $\pm$ 2.85  & 57.58 & 64.01 $\pm$ 1.53 & 66.02 $\pm$ 1.28 & 67.73 $\pm$ 0.82 \\
    \textsc{ur} & 40.77       & 58.48 $\pm$ 6.51  &63.38 $\pm$ 4.88 &66.49 $\pm$ 4.64  & 52.40 & 74.95 $\pm$ 2.15 & 78.53 $\pm$ 1.38 & 79.57 $\pm$ 1.24 \\
    \textsc{vi} & 64.67       & 68.77 $\pm$ 3.54  &69.64 $\pm$ 3.63 &71.08 $\pm$ 3.28  & 54.96 & 64.79 $\pm$ 2.33 & 69.39 $\pm$ 1.73 & 72.36 $\pm$ 1.51 \\
    \textsc{yo} & 35.48       & 53.55 $\pm$ 6.19  &58.22 $\pm$ 5.47 &65.46 $\pm$ 7.10  & -     & -               & -               & -    \\
    \textsc{zh} & 13.95       & 32.84 $\pm$ 7.10  &40.34 $\pm$ 5.32 &48.49 $\pm$ 4.30  & 63.01 & 74.15 $\pm$ 1.96 & 76.62 $\pm$ 1.39 & 79.42 $\pm$ 0.83
  \end{tabularx}
  \caption{Zero-shot (column $K=0$) and few-shot (columns $K>0$) cross-lingual transfer results on the test sets of two sequence tagging tasks NER and POS.}
  \tablabel{posnerfewshot}
\end{table*}




==> xnlipawsxfewshottable.tex <==
\begin{table}[t]
  \centering
  \tiny
  \renewcommand{\arraystretch}{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{c|ccccc}
                     &
    K=0              &
    K=1              &
    K=2              &
    K=4              &
    K=8                \\ \hline
    EN               &
    82.67            &
    -                &
    -                &
    -                &
    -                  \\
    DE               &
    70.32            &
    70.58 $\pm$ 0.36  &
    70.60 $\pm$ 0.34  &
    70.61 $\pm$ 0.39  &
    70.70 $\pm$ 0.50    \\
    FR               &
    73.57            &
    73.41 $\pm$ 0.48   &
    73.74 $\pm$ 0.46   &
    73.57 $\pm$ 0.49   &
    73.77 $\pm$ 0.44     \\
    ES               &
    73.71            &
    73.84 $\pm$ 0.40   &
    73.87 $\pm$ 0.44   &
    73.74 $\pm$ 0.48   &
    73.87 $\pm$ 0.46     \\
    RU               &
    68.70            &
    68.81 $\pm$ 0.52   &
    68.76 $\pm$ 0.54   &
    68.87 $\pm$ 0.55   &
    68.81 $\pm$ 0.77     \\
    ZH               &
    69.32            &
    69.73 $\pm$ 0.94   &
    69.75 $\pm$ 0.94   &
    70.56 $\pm$ 0.76   &
    70.62 $\pm$ 0.86     \\
    AR               &
    64.97            &
    64.75 $\pm$ 0.36   &
    64.82 $\pm$ 0.23   &
    64.82 $\pm$ 0.23   &
    64.94 $\pm$ 0.37     \\
    BG               &
    67.58            &
    68.15 $\pm$ 0.69   &
    68.19 $\pm$ 0.75   &
    68.55 $\pm$ 0.67   &
    68.32 $\pm$ 0.70     \\
    EL               &
    65.67            &
    65.64 $\pm$ 0.40   &
    65.73 $\pm$ 0.36   &
    65.80 $\pm$ 0.41   &
    66.00 $\pm$ 0.53     \\
    HI               &
    56.57            &
    56.94 $\pm$ 0.82   &
    57.07 $\pm$ 0.82   &
    57.21 $\pm$ 1.14   &
    57.82 $\pm$ 1.18     \\
    SW               &
    48.08            &
    50.33 $\pm$ 1.08   &
    50.28 $\pm$ 1.24   &
    51.08 $\pm$ 0.62   &
    51.01 $\pm$ 0.79     \\
    TH               &
    46.17            &
    49.43 $\pm$ 2.60   &
    50.08 $\pm$ 2.42   &
    51.32 $\pm$ 2.07   &
    52.16 $\pm$ 2.43     \\
    TR               &
    60.40            &
    61.02 $\pm$ 0.68   &
    61.20 $\pm$ 0.61   &
    61.35 $\pm$ 0.49   &
    61.31 $\pm$ 0.56     \\
    UR               &
    57.05            &
    57.56 $\pm$ 0.85   &
    57.83 $\pm$ 0.91   &
    58.20 $\pm$ 0.93   &
    58.67 $\pm$ 1.03     \\
    VI               &
    69.82            &
    70.04 $\pm$ 0.59   &
    70.14 $\pm$ 0.75   &
    70.23 $\pm$ 0.63   &
    70.41 $\pm$ 0.70     \\\hline\hline


    EN               &
    93.90            &
    -                &
    -                &
    -                &
    -                  \\
    DE               &
    83.80            &
    84.14 $\pm$ 0.40 &
    84.08 $\pm$ 0.42 &
    84.04 $\pm$ 0.47 &
    84.23 $\pm$ 0.66   \\

    FR               &
    86.90            &
    87.07 $\pm$ 0.27 &
    87.06 $\pm$ 0.37 &
    87.03 $\pm$ 0.31 &
    86.94 $\pm$ 0.41   \\

    ES               &
    88.25            &
    87.90 $\pm$ 0.54 &
    87.80 $\pm$ 0.56 &
    87.84 $\pm$ 0.53 &
    87.85 $\pm$ 0.75   \\

    ZH               &
    77.75            &
    77.71 $\pm$ 0.37 &
    77.63 $\pm$ 0.47 &
    77.68 $\pm$ 0.51 &
    77.82 $\pm$ 0.64   \\

    JA               &
    73.30            &
    73.78 $\pm$ 0.75 &
    73.71 $\pm$ 1.04 &
    73.48 $\pm$ 0.69 &
    73.79 $\pm$ 1.28   \\
  \end{tabular}

  \caption{Zero-shot (column K=0) and few-shot (columns K$>$0) crosslingual transfer
    results on the test
    set of XNLI (top) and PAWSX (bottom). }
  \tablabel{xnlipawsxfewshot}
\end{table}


